Analyzing Privacy Implications of Data Collection in Android Automotive OS

Modern vehicles have become sophisticated computation and sensor systems, as evidenced by advanced driver assistance systems, in-car infotainment, and autonomous driving capabilities. They collect and process vast amounts of data through various embedded subsystems. One significant player in this landscape is Android Automotive OS (AAOS), which has been integrated into over 100M vehicles and has become a dominant force in the in-vehicle infotainment market. With this extensive data collection, privacy has become increasingly crucial. The volume of data gathered by these systems raises questions about how this information is stored, used, and protected, making privacy a critical issue for manufacturers and consumers. However, very little has been done on vehicle data privacy. This paper focuses on the privacy implications of AAOS, examining the exact nature and scope of data collection and the corresponding privacy policies from the original equipment manufacturers (OEMs). We develop a novel automotive privacy analysis tool called PriDrive which employs three methodological approaches: network traffic inspection, and both static and dynamic analyses of Android images using rooted emulators from various OEMs. These methodologies are followed by an assessment of whether the collected data types were properly disclosed in OEMs and 3rd party apps' privacy policies (to identify any discrepancies or violations). Our evaluation on three different OEM platforms reveals that vehicle speed is collected at a sampling rate of roughly 25 Hz. Other properties such as model info, climate & AC, and seat data are collected in a batch 30 seconds into vehicle startup. In addition, several vehicle property types were collected without disclosure in their respective privacy policies. For example, OEM A's policies only covers 110 vehicle properties or 13.02% of the properties found in our static analysis.

==> FiguresTex/fig_getrequest.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\columnwidth]{Figures/get_request.pdf}
    \caption{Get Request made to Google Servers}
    \label{fig:get_request}
\end{figure*}

==> FiguresTex/tab_custom_oem_vhal_props.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{
%   |>{}l|
%    >{\columncolor[RGB]{255,200,200}}l|
%    >{\columncolor[RGB]{255,165,0}}l|
%    >{\columncolor[RGB]{255,255,0}}l|
%    >{\columncolor[RGB]{0,128,0}}l|
%    >{\columncolor[RGB]{0,0,255}}l|
%    >{\columncolor[RGB]{128,0,128}}l|
% }
% \hline
% \rowcolor[gray]{0.8}
% \textbf{Category} & \textbf{OEM A} & \textbf{OEM B} & \textbf{OEM C} & \textbf{OEM D} \\ \hline
% User Pref.        & 1600           & 62             & 8              & 22            \\ \hline
% Drive Assist.     & 1698           & 20             & 11             & 1             \\ \hline
% Energy            & 1076           & 9              & 0              & 1             \\ \hline
% Lighting          & 72             & 45             & 0              & 0             \\ \hline
% Diagnosis         & 1107           & 74             & 0              & 0             \\ \hline
% Climate           & 780            & 44             & 16             & 16            \\ \hline
% \end{tabular}
% \caption{Total Custom VHAL Property occurrences in an OEM emulator by category}
% \label{your-label}
% \end{table}

\begin{table}[]
\centering
\begin{tabular}{
  |>{}l|
   >{\columncolor[RGB]{255,200,200}}l|
   >{\columncolor[RGB]{255,165,0}}l|
   >{\columncolor[RGB]{255,255,0}}l|
   >{\columncolor[RGB]{0,128,0}}l|
   >{\columncolor[RGB]{0,0,255}}l|
}
\hline
\rowcolor[gray]{0.8}
\textbf{Category} & \textbf{OEM A} & \textbf{OEM B} & \textbf{OEM C} \\ \hline
User Preference        & 1600           & 62             & 8     \\ \hline
Driving Assistance     & 1698           & 20             & 11    \\ \hline
Energy and Maintenance            & 1076           & 9              & 0     \\ \hline
Lighting          & 72             & 45             & 0     \\ \hline
Diagnostics and Monitoring        & 1107           & 74             & 0     \\ \hline
Climate and Comfort          & 780            & 44             & 16    \\ \hline
\end{tabular}
\caption{Total Custom VHAL Property occurrences in an OEM emulator by category}
\label{your-label}
\end{table}

==> FiguresTex/tab_oem_permissions_vhal.tex <==
% \begin{table}[h!]
% \centering
% \caption{Number of Custom Permissions and Properties Defined by OEMs}
% \label{table:your_label}
% \begin{tabular}{lll}
% \toprule
% \makecell{Platform} & \makecell{Custom VHAL \\ Properties} & \makecell{Custom Permissions} \\
% \midrule
% % AOSP   & 3                      & 9                  \\
% \makecell{\OEM{A}}   & \makecell{753}     & \makecell{225} \\
% \makecell{\OEM{B}} & \makecell{436}    & \makecell{338} \\
% \makecell{\OEM{C}}  & \makecell{193}    & \makecell{34}  \\
% \makecell{\OEM{D}} & \makecell{156}    & \makecell{21}  \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[h!]
\centering
\caption{Number of Custom Permissions and Properties Defined by OEMs}
\label{table:unique_props_perms}
\begin{tabular}{lll}
\toprule
\makecell{Platform} & \makecell{Custom  \\ VHAL Properties} & \makecell{Custom Permissions} \\
\midrule
% AOSP   & 3                      & 9                  \\
\makecell{\OEM{A}}   & \makecell{753}     & \makecell{225} \\
\makecell{\OEM{B}} & \makecell{435}    & \makecell{338} \\
\makecell{\OEM{C}}  & \makecell{192}    & \makecell{34}  \\
\bottomrule
\end{tabular}
\end{table}

==> FiguresTex/tab_oem_vhal_props.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \rowcolor[gray]{0.8}
%   & \textbf{\OEM{A}} & \textbf{\OEM{B}} & \textbf{\OEM{C}} & \textbf{\OEM{D}} \\ \hline
% \cellcolor{red!30}A & 1600  & 62      & 8    & 22        \\ \hline
% \cellcolor{orange!30}B & 1698  & 20      & 11     & 1       \\ \hline
% \cellcolor{yellow!30}C & 1076  & 9     & 0       & 1        \\ \hline
% \cellcolor{green!30}D & 72    & 45    & 0      & 0         \\ \hline
% \cellcolor{blue!30}E & 1107  & 74    & 0      & 0         \\ \hline
% \cellcolor{purple!30}F & 780   & 44    & 16     & 16        \\ \hline
% \end{tabular}
% \caption{OEM VHAL Property occurrences by category}
% \label{your-label}
% \end{table}








==> backup/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip

